U-CREAT: Unsupervised Case Retrieval using Events extrAcTion

The task of Prior Case Retrieval (PCR) in the legal domain is about automatically citing relevant (based on facts and precedence) prior legal cases in a given query case. To further promote research in PCR, in this paper, we propose a new large benchmark (in English) for the PCR task: IL-PCR (Indian Legal Prior Case Retrieval) corpus. Given the complex nature of case relevance and the long size of legal documents, BM25 remains a strong baseline for ranking the cited prior documents. In this work, we explore the role of events in legal case retrieval and propose an unsupervised retrieval method-based pipeline U-CREAT (Unsupervised Case Retrieval using Events Extraction). We find that the proposed unsupervised retrieval method significantly increases performance compared to BM25 and makes retrieval faster by a considerable margin, making it applicable to real-time case retrieval systems. Our proposed system is generic, we show that it generalizes across two different legal systems (Indian and Canadian), and it shows state-of-the-art performance on the benchmarks for both the legal systems (IL-PCR and COLIEE corpora).

==> acknowledgement.tex <==
\section*{Acknowledgements} 
%\subsubsection{Acknowledgements} 
Please place your acknowledgments at
the end of the paper, preceded by an unnumbered run-in heading (i.e.
3rd-level heading).

==> events.tex <==
% \subsection{Event Extraction} \label{sec:events}
% A story or an incident is best described in the sequence of events. These events are narrative and form a partially ordered set called a narrative event chain \cite{Event_Chains}. In every sentence, the most important word, predicate, conveys the happening at a given instance, and a set of ordered predicates explain the story sequentially. However, a set of ordered predicates does not reflect the nature of the subject, object, and relation. In the legal domain, the role of subject and object is significant as they share a contextual relationship with the action\cite{Event_chains_participants}. Therefore, we use a triplet of subject, predicate and object to capture the core meaning of the sentence. We refer to this triplet as an event. First, the text is cleaned and then parsed using Spacy's \cite{Spacy} Dependency parsing pipeline to extract the word's dependencies and parts of speech.



% <Sub-Heading 1: Preprocessing>

% Legal documents have a period after the initials of those involved in that case. The period is also present with abbreviations like "Dr", "Mr", "Mrs", "vs",  "addl", and many more. The surnames with single letters and periods and the standard abbreviations used in the legal domain were manually listed and removed during the preprocessing. The regular expressions were used to eliminate other unwanted characters and symbols in the text.

% <Sub-Heading 2: Dependency Parsing>

% Dependency parsing represents the grammatical structure and dependency relationship of words in a sentence. The head of the sentence has no dependency and is called the root. Other words like the subject, object, preposition, and adverb are linked to the root. The dependencies mapped in a directed graph representation constitute nodes formed by the words of the sentence, and the edges are the relationships between the dependents and the head of the given sentence. It also describes the syntactic roles of each word. 
% The directed graph formed by the dependency parser has the properties of a tree. It can be traversed in different directions to extract relationships. All kinds of relations like lefts, rights, children and subtrees are available to navigate the parse tree. 

% <Add spacy pipe line picture>

% <Add an example showing the mapping of verb with other words>

% Sentences in the text are parsed through the dependency parser to extract the list of verbs. These verbs form the root of the dependency tree. The lefts of each verb are examined to find the subjects with syntactic dependency relationships like nsubj, nsubjpass, and csubj. The rights of a verb with relationships like dobj, pobj, and dative indicate the object's presence. Further, the lefts and rights are examined for conjunctions and compounds to get all the possible subjects and objects. Finally, named entities such as person names, organizations, locations and so on were extracted and replaced with a generic tag like "<PERSON>", "<ORG>", "<LOCATION>" while the remaining words were lemmatized to make the event generic. 

% <Show examples of events generated in different sentences>

% Events have an essential role in establishing the relationship between the case and the precedent. If a case has a precedent, both are related based on the nature of the cases, evidence, and judgement. The events in a prior case form a basis for the arguments and judgements in such similar cases. Table [?] shows the similarity of events between two cases of which one is citing the other.


% <Put a table which shows common events between a case and its citations>





